A Robust Pedestrian Detection Approach for Autonomous Vehicles

Nowadays, utilizing Advanced Driver-Assistance Systems (ADAS) has absorbed a huge interest as a potential solution for reducing road traffic issues. Despite recent technological advances in such systems, there are still many inquiries that need to be overcome. For instance, ADAS requires accurate and real-time detection of pedestrians in various driving scenarios. To solve the mentioned problem, this paper aims to fine-tune the YOLOv5s framework for handling pedestrian detection challenges on the real-world instances of Caltech pedestrian dataset. We also introduce a developed toolbox for preparing training and test data and annotations of Caltech pedestrian dataset into the format recognizable by YOLOv5. Experimental results of utilizing our approach show that the mean Average Precision (mAP) of our fine-tuned model for pedestrian detection task is more than 91 percent when performing at the highest rate of 70 FPS. Moreover, the experiments on the Caltech pedestrian dataset samples have verified that our proposed approach is an effective and accurate method for pedestrian detection and can outperform other existing methodologies.

==> temp.tex <==
Other Pedestrian Detection Approaches:

Please take a look at following papers with code implementations. These are the codes implemented for Ped. Detection on Caltech.

1: Learning Efficient Single-stage Pedestrian Detectors by Asymptotic Localization Fitting (2018)
- Link to the paper: https://paperswithcode.com/paper/learning-efficient-single-stage-pedestrian
- Link to the code: https://github.com/VideoObjectSearch/ALFNet

2: Repulsion Loss: Detecting Pedestrians in a Crowd (2018)
- Link to the paper: https://arxiv.org/pdf/1711.07752v2.pdf
- Link to the code: $https://github.com/bailvwangzi/repulsion_loss_ssd$

3: Part-Level Convolutional Neural Networks for Pedestrian Detection (2015)
- Link to the paper: https://arxiv.org/pdf/1810.00689v1.pdf
- Link to the code: https://github.com/iyyun/Part-CNN

4: A Unified Multi-scale Deep Convolutional Neural Network for Fast Object Detection (2016)
- Link to the paper: https://arxiv.org/pdf/1607.07155v1.pdf
- Link to the code: https://github.com/zhaoweicai/mscnn

5: Illuminating Pedestrians via Simultaneous Detection & Segmentation (2017)
- Link to the paper: https://arxiv.org/pdf/1706.08564v1.pdf
- Link to the code: https://github.com/garrickbrazil/SDS-RCNN
